SCGNet-Stacked Convolution with Gated Recurrent Unit Network for Cyber Network Intrusion Detection and Intrusion Type Classification

Intrusion detection system (IDS) is a piece of hardware or software that looks for malicious activity or policy violations in a network. It looks for malicious activity or security flaws on a network or system. IDS protects hosts or networks by looking for indications of known attacks or deviations from normal behavior (Network-based intrusion detection system, or NIDS for short). Due to the rapidly increasing amount of network data, traditional intrusion detection systems (IDSs) are far from being able to quickly and efficiently identify complex and varied network attacks, especially those linked to low-frequency attacks. The SCGNet (Stacked Convolution with Gated Recurrent Unit Network) is a novel deep learning architecture that we propose in this study. It exhibits promising results on the NSL-KDD dataset in both task, network attack detection, and attack type classification with 99.76% and 98.92% accuracy, respectively. We have also introduced a general data preprocessing pipeline that is easily applicable to other similar datasets. We have also experimented with conventional machine-learning techniques to evaluate the performance of the data processing pipeline.

==> Run_This_Examplebib <==
@misc{1_omalley2019kerastuner,
    title        = {KerasTuner},
    author       = {O'Malley, Tom and Bursztein, Elie and Long, James and Chollet, Fran\c{c}ois and Jin, Haifeng and Invernizzi, Luca and others},
    year         = 2019,
    howpublished = {\url{https://github.com/keras-team/keras-tuner}}
}

@article{2_li2017hyperband,
  title={Hyperband: A novel bandit-based approach to hyperparameter optimization},
  author={Li, Lisha and Jamieson, Kevin and DeSalvo, Giulia and Rostamizadeh, Afshin and Talwalkar, Ameet},
  journal={The Journal of Machine Learning Research},
  volume={18},
  number={1},
  pages={6765--6816},
  year={2017},
  publisher={JMLR. org}
}

@inproceedings{1.1_chung2015heuristic,
  title={A heuristic approach to enhance the performance of intrusion detection system using machine learning algorithms},
  author={Chung, Sunook and Kim, Kwangjo},
  booktitle={Proceedings of the Korea Institutes of Information Security and Cryptology Conference (CISC-W’15)},
  year={2015}
}

@inproceedings{2.2_huang2017densely,
  title={Densely connected convolutional networks},
  author={Huang, Gao and Liu, Zhuang and Van Der Maaten, Laurens and Weinberger, Kilian Q},
  booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
  pages={4700--4708},
  year={2017}
}

@article{3_laghrissi2021intrusion,
  title={Intrusion detection systems using long short-term memory (LSTM)},
  author={Laghrissi, FatimaEzzahra and Douzi, Samira and Douzi, Khadija and Hssina, Badr},
  journal={Journal of Big Data},
  volume={8},
  number={1},
  pages={65},
  year={2021},
  publisher={Springer}
}

@article{4_ma2017learning,
  title={Learning traffic as images: A deep convolutional neural network for large-scale transportation network speed prediction},
  author={Ma, Xiaolei and Dai, Zhuang and He, Zhengbing and Ma, Jihui and Wang, Yong and Wang, Yunpeng},
  journal={Sensors},
  volume={17},
  number={4},
  pages={818},
  year={2017},
  publisher={MDPI}
}

@article{5_kunang2021attack,
  title={Attack classification of an intrusion detection system using deep learning and hyperparameter optimization},
  author={Kunang, Yesi Novaria and Nurmaini, Siti and Stiawan, Deris and Suprapto, Bhakti Yudho},
  journal={Journal of Information Security and Applications},
  volume={58},
  pages={102804},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{6_tavallaee2009detailed,
  title={A detailed analysis of the KDD CUP 99 data set},
  author={Tavallaee, Mahbod and Bagheri, Ebrahim and Lu, Wei and Ghorbani, Ali A},
  booktitle={2009 IEEE symposium on computational intelligence for security and defense applications},
  pages={1--6},
  year={2009},
  organization={Ieee}
}

@inproceedings{7_divekar2018benchmarking,
  title={Benchmarking datasets for anomaly-based network intrusion detection: KDD CUP 99 alternatives},
  author={Divekar, Abhishek and Parekh, Meet and Savla, Vaibhav and Mishra, Rudra and Shirole, Mahesh},
  booktitle={2018 IEEE 3rd International Conference on Computing, Communication and Security (ICCCS)},
  pages={1--8},
  year={2018},
  organization={IEEE}
}

@article{8_tama2019tse,
  title={TSE-IDS: A two-stage classifier ensemble for intelligent anomaly-based intrusion detection system},
  author={Tama, Bayu Adhi and Comuzzi, Marco and Rhee, Kyung-Hyune},
  journal={IEEE access},
  volume={7},
  pages={94497--94507},
  year={2019},
  publisher={IEEE}
}

@article{9_ma2016hybrid,
  title={A hybrid spectral clustering and deep neural network ensemble algorithm for intrusion detection in sensor networks},
  author={Ma, Tao and Wang, Fen and Cheng, Jianjun and Yu, Yang and Chen, Xiaoyun},
  journal={Sensors},
  volume={16},
  number={10},
  pages={1701},
  year={2016},
  publisher={MDPI}
}

@article{10_vasilomanolakis2015taxonomy,
  title={Taxonomy and survey of collaborative intrusion detection},
  author={Vasilomanolakis, Emmanouil and Karuppayah, Shankar and M{\"u}hlh{\"a}user, Max and Fischer, Mathias},
  journal={ACM Computing Surveys (CSUR)},
  volume={47},
  number={4},
  pages={1--33},
  year={2015},
  publisher={ACM New York, NY, USA}
}

@inproceedings{11_sukumar2018network,
  title={Network intrusion detection using improved genetic k-means algorithm},
  author={Sukumar, JV Anand and Pranav, I and Neetish, MM and Narayanan, Jayasree},
  booktitle={2018 international conference on advances in computing, communications and informatics (ICACCI)},
  pages={2441--2446},
  year={2018},
  organization={IEEE}
}

@article{12_naseer2018enhanced,
  title={Enhanced network anomaly detection based on deep neural networks},
  author={Naseer, Sheraz and Saleem, Yasir and Khalid, Shehzad and Bashir, Muhammad Khawar and Han, Jihun and Iqbal, Muhammad Munwar and Han, Kijun},
  journal={IEEE access},
  volume={6},
  pages={48231--48246},
  year={2018},
  publisher={IEEE}
}

@article{13_kasongo2020deep,
  title={A deep learning method with wrapper based feature extraction for wireless intrusion detection system},
  author={Kasongo, Sydney Mambwe and Sun, Yanxia},
  journal={Computers \& Security},
  volume={92},
  pages={101752},
  year={2020},
  publisher={Elsevier}
}


@article{14_li2020building,
  title={Building auto-encoder intrusion detection system based on random forest feature selection},
  author={Li, XuKui and Chen, Wei and Zhang, Qianru and Wu, Lifa},
  journal={Computers \& Security},
  volume={95},
  pages={101851},
  year={2020},
  publisher={Elsevier}
}

@article{15_chkirbene2020tidcs,
  title={TIDCS: A dynamic intrusion detection and classification system based feature selection},
  author={Chkirbene, Zina and Erbad, Aiman and Hamila, Ridha and Mohamed, Amr and Guizani, Mohsen and Hamdi, Mounir},
  journal={IEEE Access},
  volume={8},
  pages={95864--95877},
  year={2020},
  publisher={IEEE}
}

@article{16_boukhalfa2020lstm,
  title={LSTM deep learning method for network intrusion detection system},
  author={Boukhalfa, Alaeddine and Abdellaoui, Abderrahim and Hmina, Nabil and Chaoui, Habiba},
  journal={International Journal of Electrical and Computer Engineering},
  volume={10},
  number={3},
  pages={3315},
  year={2020},
  publisher={IAES Institute of Advanced Engineering and Science}
}

@article{17_pooja2021evaluating,
  title={Evaluating neural networks using Bi-Directional LSTM for network IDS (intrusion detection systems) in cyber security},
  author={Pooja, TS and Shrinivasacharya, Purohit},
  journal={Global Transitions Proceedings},
  volume={2},
  number={2},
  pages={448--454},
  year={2021},
  publisher={Elsevier}
}

@article{18_chawla2002smote,
  title={SMOTE: synthetic minority over-sampling technique},
  author={Chawla, Nitesh V and Bowyer, Kevin W and Hall, Lawrence O and Kegelmeyer, W Philip},
  journal={Journal of artificial intelligence research},
  volume={16},
  pages={321--357},
  year={2002}
}

 @misc{19_b_2020, title={Confusion matrix, accuracy, precision, recall, F1 score}, url={https://medium.com/analytics-vidhya/confusion-matrix-accuracy-precision-recall-f1-score-ade299cf63cd}, journal={Medium}, publisher={Analytics Vidhya}, author={B, Harikrishnan N}, year={2020}, month={Jun}} 

